K-Core Minimization: A Game Theoretic Approach

K-cores are maximal induced subgraphs where all vertices have degree at least k. These dense patterns have applications in community detection, network visualization and protein function prediction. However, k-cores can be quite unstable to network modifications, which motivates the question: How resilient is the k-core structure of a network, such as the Web or Facebook, to edge deletions? We investigate this question from an algorithmic perspective. More specifically, we study the problem of computing a small set of edges for which the removal minimizes the $k$-core structure of a network. This paper provides a comprehensive characterization of the hardness of the k-core minimization problem (KCM), including innaproximability and fixed-parameter intractability. Motivated by such a challenge in terms of algorithm design, we propose a novel algorithm inspired by Shapley value -- a cooperative game-theoretic concept -- that is able to leverage the strong interdependencies in the effects of edge removals in the search space. As computing Shapley values is also NP-hard, we efficiently approximate them using a randomized algorithm with probabilistic guarantees. Our experiments, using several real datasets, show that the proposed algorithm outperforms competing solutions in terms of k-core minimization while being able to handle large graphs. Moreover, we illustrate how KCM can be applied in the analysis of the k-core resilience of networks.

==> extra.tex <==
\begin{comment}
%computeVS
\begin{algorithm}[t]
\caption{computeVS(e)}
\begin{algorithmic}[1]
\STATE $S \leftarrow \{N,M\}$
\IF{$M \in N.critNeighbors$}
\STATE $\textit{VS}.add(N)$
\ENDIF
\IF{$N \in M.critNeighbors \And M.critDegree = M.coreNumber$}
\STATE $\textit{VS}.add(M)$
\ENDIF
\WHILE{$S \not = \emptyset$ }
\STATE $currNode \in S$
\FOR{$node K \in currNode.neighbors$}
\IF{$K \not \in \textit{VS}\And K.critDegree - |K.vulnerableNeighbour|<K.coreNumber $}
\STATE $\textit{VS}.add(K)$
\STATE $S.add(K)$
\ENDIF
\ENDFOR
\STATE $S.remove(K)$
\ENDWHILE
\end{algorithmic}
\label{computeVS}
\end{algorithm}
\end{comment}

\begin{comment}
%The Equivalent Set Algorithm
\begin{algorithm}[t]
\caption{Equivalent Set (Greedy Cut)}
\begin{algorithmic}[1]
\STATE $max \leftarrow -\infty$
\STATE $\textit{ES} \leftarrow \emptyset$
\FOR{$node N \in graph G$}
\IF{$N.critDegree = N.coreNumber \And N \not \in \textit{ES}$}
\STATE $\textit{VS} \leftarrow\emptyset$
\STATE $edgeNM \in N.critEdges()$
\STATE computeVS($N,M$)
\STATE $\textit{ES} \leftarrow \textit{ES} \bigcup \textit{VS}$
\IF{$|\textit{VS}|  > max $}
\STATE $max \leftarrow |\textit{VS}|$
\STATE $candidate \leftarrow edgeNM)$
\ENDIF
\ENDIF
\ENDFOR
\STATE $G.remove(candidate)$
\STATE localUpdate($candidate.first$)
\IF{$candidate.second.critDegree < its\; coreNumber$}
\STATE localUpdate($candidate.second$)
\ENDIF
\end{algorithmic}
\label{vulnerable}
\end{algorithm}

%The Equivalent Set Algorithm
\begin{algorithm}[t]
\caption{Equivalent Set (Greedy Cut)}
\begin{algorithmic}[1]
\STATE $max \leftarrow -\infty$
\STATE $\textit{ES} \leftarrow \emptyset$
\FOR{$node N \in graph G$}
\IF{$N.critDegree = N.coreNumber \And N \not \in \textit{ES}$}
\STATE $\textit{VS} \leftarrow\emptyset$
\STATE $edgeNM \in N.critEdges()$
\STATE computeVS($N,M$)
\STATE $\textit{ES} \leftarrow \textit{ES} \bigcup \textit{VS}$
\IF{$|\textit{VS}|  > max $}
\STATE $max \leftarrow |\textit{VS}|$
\STATE $candidate \leftarrow edgeNM)$
\ENDIF
\ENDIF
\ENDFOR
\STATE $G.remove(candidate)$
\STATE localUpdate($candidate.first$)
\IF{$candidate.second.critDegree < its\; coreNumber$}
\STATE localUpdate($candidate.second$)
\ENDIF
\end{algorithmic}
\label{vulnerable}
\end{algorithm}
\end{comment}



\begin{comment}
%localUpdate
\begin{algorithm}[t]
\caption{localUpdate($N$)}
\begin{algorithmic}[1]
\STATE $N.coreNumber\text{ -- } \text{--}$
\STATE $S \leftarrow \{N\}$
\WHILE{$S \not = \emptyset$}
\STATE $currNode \in S$
\FOR{$node K \in currNode.neighbors$}
\IF{$K.critDegree < K.coreNumber$}
\STATE $K.coreNumber\text{ -- } \text{--}$
\STATE $S.add(K)$
\ENDIF
\ENDFOR
\IF{$currNode.coreNumber < k$}
\STATE $G.remove(currNode)$
\ENDIF
\STATE $S.remove(currNode)$
\ENDWHILE
\end{algorithmic}
\label{computeVS}
\end{algorithm}
\end{comment}
